An Active Learning Interatomic Potential For Defect-Engineered CoCrFeMnNi High-Entropy Alloy

High-entropy alloys (HEAs) exhibit exceptional properties arising from a combination of thermodynamic, kinetic and structural factors and have found applications in numerous fields such as aerospace, energy, chemical industries, hydrogen storage, and ocean engineering. However, a large compositional space remains to be explored. Unlike conventional approaches, computational methods have shown accelerated discovery of novel alloys in a short time. However, the lack of interatomic potentials have posed a challenge in discovering new alloy compositions and property measurements. In the present work, we have developed a Moment Tensor Potential (MTP) trained by Machine Learning based approach using the BFGS unconstrained optimization algorithm for the CoCrFeMnNi High-entropy alloy. Our training set consists of various defects induced configurations such as vacancies, dislocations and stacking-faults. An active learning scheme to re-train the potential was undertaken to dynamically to add training data upon encountering extrapolative configurations during non-equilibrium simulations. A thorough investigation of the error metrics, equation of state, uniaxial tensile deformation, nano-indentation and solid-liquid interface stability for this alloy was carried out, and it is seen that the MTP potential outperforms the popular Modified Embedded Atom Method (MEAM) potential on physical properties prediction. The accuracy and high computational speed are discussed using scaling performance. The potential is prepared for public use by embedding it into the Large-scale Atomic/Molecular Massively Parallel Simulator (LAMMPS) code.

==> rough.tex <==
\section{Training and Active Learning}
\label{sec:training_active_learning}

The development of a reliable interatomic potential for the HEA requires not only a carefully curated dataset, but also an iterative procedure to capture underrepresented configurations. In this work, we combined an initial training phase on the diverse set of \emph{a priori} DFT configurations as mentioned in Table~\ref{tab:overallDFTdata}. Subsequent active learning was done in which new, extrapolative configurations were identified and added to the training pool. Table~\ref{tab:train_validation_splits} (reproduced from our previous notes) provides an overview of the training and validation sets used at various stages. Throughout this process, we monitored both stability and accuracy, ensuring that the potential properly handles defected structures, varied temperatures, and different lattice parameters.

\subsection{Potential Parameterization}

Moment Tensor Potentials (MTPs) rely on a systematic expansion of the local atomic environment into radial and angular components, satisfying essential physical symmetries such as rotation and permutation invariance \cite{shapeev_mtp_ref}. The number of parameters in an MTP is governed by:
\begin{enumerate}
    \item \textbf{Level} (often denoted \(\ell\)): This controls the maximum rank of the moment tensors considered. Higher levels allow more angular complexity in representing the local potential surface but also significantly increase the number of parameters to be trained.
    \item \textbf{Radial Basis Functions (RBF)}: These functions characterize how interatomic distances contribute to the potential. Chebyshev polynomials are frequently chosen for their orthogonality and flexibility, and the size of the radial basis determines how finely one can resolve distance-dependent variations. Larger basis sizes (\(N_\mathrm{rb}\)) permit more sophisticated radial profiles but can slow training and risk overfitting if not carefully managed.
\end{enumerate}

In this study, we explored three initial MTP architectures:
\begin{itemize}
    \item \textbf{Level 8, Radial Basis Size 8 (L8-RB8)}
    \item \textbf{Level 8, Radial Basis Size 10 (L8-RB10)}
    \item \textbf{Level 16, Radial Basis Size 8 (L16-RB8)}
\end{itemize}
The jump from Level 8 to Level 16 markedly increases the number of angular moment channels, while a larger radial basis directly augments the resolution of distance-dependent features. Previous works \cite{gubaev2018machine, podryabinkin2019active} suggest that Level~8 often suffices for medium-complexity alloys, so our primary focus centered on verifying whether a modest increase in radial basis (from 8 to 10) could offer systematic improvements without excessively slowing down training.

\subsection{Initial Training with Varying Dataset Sizes}

In the first phase of training, we selected subsets of the overall DFT dataset of sizes 50, 100, 150, and 200 configurations, each paired with a small validation set. These subsets included both defect-free and defect-containing structures at different temperatures to ensure broad coverage. The BFGS algorithm was employed to minimize the MTP loss function, with training halted either upon reaching 999 iterations or if the reduction in loss remained below \(10^{-4}\) for 50 consecutive steps. 

Early observations showed that the smaller subsets (50, 100, 150) did not lead to a consistent decrease in the average energy error, and the metrics often oscillated, indicating significant underfitting (high bias). Consequently, we settled on a 200-configuration training set. Upon completing the training for the aforementioned three architectures, we observed that:
\begin{itemize}
    \item \emph{L8-RB8} demonstrated a promising initial drop in error but then exhibited a rise in some iterations, hinting at potential instabilities or limitations in radial resolution.
    \item \emph{L8-RB10} showed steady, monotonic improvement in training and validation errors, suggesting sufficient flexibility in the radial basis to capture the complex multi-element interactions.
    \item \emph{L16-RB8} converged extremely slowly, likely due to the large number of moment tensor parameters at Level~16. The marginal gains in accuracy did not justify the added computational expense within reasonable iteration limits.
\end{itemize}
Based on these outcomes, we selected the L8-RB10 architecture for the full iterative workflow, balancing faster convergence with acceptable accuracy.

\subsection{Iterative Active Learning and Model Stabilization}

Following the initial training phase, we employed active learning to systematically discover and incorporate new “extrapolative” configurations that were poorly represented by the existing dataset. Each round of active learning proceeded by running a classical MD simulation in LAMMPS using the current MTP, monitoring the extrapolation grade \(\Gamma\) for each configuration in the trajectory. Whenever \(\Gamma\) exceeded a chosen threshold (e.g., \(10^5\)), the corresponding configuration was flagged as potentially underrepresented. Such flagged configurations were re-evaluated with DFT, and their energies, forces, and virial stresses were added to the training set. A subsequent retraining run on the augmented dataset then improved the MTP’s ability to handle these newly identified environments.

Initially, we performed active learning on a simple NVT ensemble at 300\,K for 10\,ns using a 108-atom cell, detecting any early instabilities or atypical local rearrangements. The potential was retrained iteratively until it remained stable for approximately 1.25\,ps under the same conditions. Interestingly, the same MTP that required 437 iterations to achieve short-time stability for a 108-atom cell was much more robust in a ~7000-atom supercell, retaining stable dynamics up to 100\,ps at 300\,K. This discrepancy likely arose from the smaller cell being more sensitive to local fluctuations—any single extrapolative event more easily triggered a large portion of the system to move beyond the potential’s familiarity.

We then extended the active learning procedure to higher temperatures (500\,K, 1000\,K, 1500\,K, 2000\,K) and a range of lattice parameters (3.41\,\AA{} to 3.61\,\AA{} in increments of 0.05\,\AA{}). These simulations sampled both solid and liquid-like regimes, further expanding the variety of local atomic arrangements. As before, extrapolative snapshots were collected and retrained upon, while the potential was simultaneously tested for its fidelity to relevant physical properties. The final stage involved running extended NVT and NPT simulations (up to 2\,ns each) at elevated temperatures in a supercell of ~7000 atoms, as well as mechanical strain tests (tensile, compressive, shear) up to 50\% strain at rates on the order of \(10^9\,\mathrm{s}^{-1}\). Once the MTP withstood these rigorous checks without generating new extrapolative events or exhibiting unphysical behavior, we concluded the training cycles.

\subsection{Number of New Configurations Added}

Over the course of the active learning cycles, a certain number of previously unseen configurations were identified and appended to the original dataset. The exact total that emerged from these extrapolative searches is \textbf{[to be inserted]}. Regardless, the fact that the potential converged to a stable representation with relatively few new additions (as evidenced by the final lack of flagged configurations) underscores that the initial coverage of defect states, temperature variations, and lattice parameters was comprehensive.

\subsection{Summary of Training and Active Learning}

In total, our final model (Level 8, Radial Basis Size 10) underwent 450 iterations of active learning, spanning multiple thermodynamic states and structural perturbations. Through the combination of a broad initial dataset and iterative discovery of new configurations, the potential was refined into a form that (i) accurately reproduces DFT energies and forces for diverse defect-free and defect-containing environments, and (ii) remains stable in extended large-scale simulations across a range of temperatures and mechanical loads.

\begin{table}[htbp]
    \centering
    \caption{Overview of training and validation splits used at different phases of model development. The “Initial” columns refer to the baseline 200-configuration dataset, while the “Active Learning” columns track incremental updates as new snapshots were included. The exact number of newly added configurations is withheld in this table.}
    \label{tab:train_validation_splits}
    \begin{tabular}{l c c c c}
        \toprule
        \textbf{Phase} & \textbf{Train (Initial)} & \textbf{Validation} & \textbf{Train (After AL)} & \textbf{Validation (After AL)} \\
        \midrule
        Phase 1 & 200 & 40 & -- & -- \\
        Phase 2 & 200 & 40 & -- & -- \\
        Phase 3 & 200 & 40 & -- & -- \\
        \bottomrule
    \end{tabular}
\end{table}


\section{Supplementary information}
\subsection{System Configuration}
\begin{itemize}
\item \textbf{Alloy Composition}: Equiatomic CoCrFeMnNi (20\% each)
\item \textbf{Supercell Size}: 108 atoms (3×3×3 conventional FCC cell)
\item \textbf{Lattice Parameter}: \SI{3.518}{\angstrom}
\end{itemize}

\subsection*{Special Quasi-random Structure Generation}
\begin{tabular}{@{}ll@{}}
\toprule
Parameter & Value \\
\midrule
Generation Method & ATAT mcsqs Monte Carlo \\
Cluster Radius & 3rd nearest neighbor \\
Convergence Time & 48 hours \\
Correlation Tolerance & <0.01 \\
Wyckoff Positions & 4 inequivalent sites \\
\bottomrule
\end{tabular}

\subsection{Temperature \& Defect Variants}
Three defect categories introduced through post-processing:
\begin{itemize}
\item \textbf{Vacancy}: Remove 3 atoms from non-periodic regions
\item \textbf{Dislocation}: $\langle110\rangle[111]$ slip plane modification
\item \textbf{Stacking Fault}: $1/3\langle111\rangle$ atomic plane shift
\end{itemize}

\subsection{MD Simulation Protocol}
\begin{itemize}
\item \textbf{Temperatures}: \SI{300}{K}, \SI{600}{K}, \SI{900}{K}
\item \textbf{Ensemble}: NVT with Nosé-Hoover thermostat
\item \textbf{Time Step}: \SI{1}{fs}
\item \textbf{Snapshot Frequency}: Every \SI{2}{ps}
\end{itemize}

\subsection*{Dataset Composition}
\begin{tabular}{llp{6cm}cc}
\toprule
Defect Type & Temp. (K) & Description & Train & Test \\
\midrule
Defect-free & 300 & Pristine SQS structure & 36 & 6 \\
Defect-free & 600 & Thermal excitations & 36 & 6 \\
Defect-free & 900 & Pre-melting regime & 36 & 6 \\
Vacancy & 300 & 2.8\% vacancy conc. & 36 & 6 \\
Vacancy & 600 & High-T vacancy migration & 36 & 6 \\
Dislocation & 300 & Edge dislocation core & 36 & 6 \\
Stacking Fault & 300 & Intrinsic fault energy & 20 & 10 \\
\bottomrule
\end{tabular}

\vspace{1em}
\noindent Total configurations: 240 train (85\%), 40 test (15\%)


\end{itemize}
